RiskReason: A Benchmark for Verifiable Financial Risk Reasoning

Robust financial-risk inference requires more than mathematical correctness. Models must accurately apply conditional rules, maintain evolving financial states, and make decisions that respect operational constraints. This work introduces RiskReason, a benchmark for verifiable financial-risk reasoning that spans diverse risk-management mechanisms. The benchmark includes Standard tasks, which assess individual financial mechanisms, and Long-horizon tasks, which combine multiple mechanisms through extended dependencies. Each task provides reference outcomes, formal specifications, reasoning annotations, and dependency representations to support systematic analysis of model performance. Eleven model configurations are evaluated using strict single-attempt accuracy, complemented by structural and qualitative failure analyses. The strongest configurations achieve 80.0--90.2\% overall accuracy, with several maintaining high performance on composed financial scenarios. However, analysis of failures reveals incorrect risk decisions despite accurate intermediate calculations, inconsistent propagation of financial states, and remediation actions that violate binding constraints. In contrast, some strict evaluation failures result from incomplete reporting rather than incorrect financial conclusions. These findings indicate that aggregate accuracy alone is insufficient to characterize financial-risk reasoning reliability and motivate evaluations that distinguish numerical correctness, state consistency, constraint satisfaction, and decision validity.

==> figures/RiskReason_risk_domain_figure.tex <==
% Conceptual benchmark overview: financial domains and an example mechanism chain.
% Requires \usepackage{tikz} and \usetikzlibrary{arrows.meta,positioning}.
\begin{figure*}[t]
\centering
\begin{tikzpicture}[
  x=1cm,y=1cm,
  riskdomain/.style={draw=blue!48!black,fill=blue!4,rounded corners=2.5pt,
    line width=.55pt,text width=2.45cm,minimum width=2.60cm,minimum height=1.06cm,
    align=center,inner sep=3pt,font=\footnotesize},
  stage/.style={draw=teal!57!black,fill=teal!5,rounded corners=2.5pt,
    line width=.6pt,text width=2.84cm,minimum height=1.55cm,
    align=center,inner sep=2.5pt,font=\footnotesize},
  steparrow/.style={-{Stealth[length=2mm,width=1.3mm]},draw=black!47,line width=.7pt},
  sectionlabel/.style={anchor=west,font=\sffamily\bfseries\scriptsize,text=black!70},
]
  % Coverage is a taxonomy, not a single mandatory reasoning chain.
  \node[sectionlabel] at (0,5.18) {FINANCIAL-RISK DOMAINS COVERED};
  \node[riskdomain] (d1) at (1.42,4.40) {\textbf{Market}\\[-1pt]{\scriptsize Valuation and shocks}};
  \node[riskdomain] (d2) at (4.31,4.40) {\textbf{Credit}\\[-1pt]{\scriptsize Default and recovery}};
  \node[riskdomain] (d3) at (7.20,4.40) {\textbf{Liquidity}\\[-1pt]{\scriptsize Cash and funding}};
  \node[riskdomain] (d4) at (10.09,4.40) {\textbf{Collateral}\\[-1pt]{\scriptsize Margin and eligibility}};
  \node[riskdomain] (d5) at (12.98,4.40) {\textbf{Counterparty}\\[-1pt]{\scriptsize Exposure and netting}};
  \node[riskdomain] (d6) at (15.87,4.40) {\textbf{Capital}\\[-1pt]{\scriptsize Leverage and adequacy}};
  \draw[black!16,line width=.5pt] (0,3.65)--(17.32,3.65);

  % Only one representative pathway, long-001. Not all tasks traverse all domains.
  \node[sectionlabel] at (0,3.28) {ILLUSTRATIVE LONG-HORIZON PATHWAY: \texttt{long-001}};
  \node[stage] (s1) at (1.52,2.22) {\textbf{Market shock}\\[2pt]{\scriptsize Yield rises 120 bp}\\[-1pt]{\scriptsize Bond loss: \$3.744M}};
  \node[stage] (s2) at (5.02,2.22) {\textbf{Collateral}\\[2pt]{\scriptsize Value declines}\\[-1pt]{\scriptsize Margin call: \$3.744M}};
  \node[stage] (s3) at (8.52,2.22) {\textbf{Liquidity}\\[2pt]{\scriptsize Cash after call: \$0.256M}\\[-1pt]{\scriptsize Below \$1.5M floor}};
  \node[stage] (s4) at (12.02,2.22) {\textbf{Funding action}\\[2pt]{\scriptsize Credit-line draw: \$1.244M}\\[-1pt]{\scriptsize Cash floor restored}};
  \node[stage] (s5) at (15.52,2.22) {\textbf{Leverage test}\\[2pt]{\scriptsize Debt/equity: $4.0372\times$}\\[-1pt]{\scriptsize Exceeds $4.0\times$ ceiling}};
  \foreach \a/\b in {s1/s2,s2/s3,s3/s4,s4/s5} {
    \draw[steparrow] (\a.east) -- (\b.west);
  }

  \node[draw=black!19,fill=black!3,rounded corners=2pt,
        minimum width=17.20cm,minimum height=.45cm,align=center,
        font=\footnotesize] at (8.52,.70)
    {\textbf{Final assessment:} liquidity requirement satisfied; leverage constraint breached};
\end{tikzpicture}
\caption{RiskReason's principal financial-risk domains and an illustrative chain of interacting mechanisms. The lower pathway summarizes the evaluated \texttt{long-001} scenario: a market shock affects collateral, triggers a liquidity response, and changes leverage compliance. The pathway is an example, not a required sequence across tasks or an exhaustive depiction of the benchmark's domains.}
\Description{At the top are six separate domain boxes: Market, Credit, Liquidity, Collateral, Counterparty, and Capital. Below, an example long-horizon chain flows from market shock to collateral margin call to cash shortfall to credit-line borrowing and a breached leverage ceiling. The final assessment states that liquidity is satisfied but leverage is breached.}
\label{fig:risk-interactions}
\end{figure*}


==> figures/fig_outcomes.tex <==
% Generated from the source grading JSON files. Only recorded pass counts as exact success.
\begin{figure*}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
    xbar stacked, bar width=7.2pt, width=0.92\textwidth, height=10.2cm,
    xmin=0, xmax=100, ymin=0.4, ymax=11.6,
    xtick={0,20,40,60,80,100}, ytick={1,...,11},
    yticklabels={Qwen2.5-7B-Instruct,DianJin-R1-7B,Fin-o1-8B,DeepSeek-R1-Distill-32B,Phi-4-Reasoning-Plus,Gemini 3.1 Pro Preview,Gemini 3.8 Flash,GPT-6 Luna,GPT-6 Sol,GPT-6 Astra,Claude Sonnet 5.5},
    yticklabel style={font=\scriptsize}, xticklabel style={font=\scriptsize},
    xlabel={Share of evaluated tasks (\%)}, xlabel style={font=\small},
    xmajorgrids, grid style={black!12}, axis line style={black!30}, tick align=outside,
    legend columns=5, legend style={at={(0.5,1.04)}, anchor=south, draw=none, font=\scriptsize, /tikz/every even column/.append style={column sep=5pt}},
]
\addplot+[fill=domc,draw=white,line width=0.25pt] coordinates {
 (90.24390,11)
 (88.23529,10)
 (87.25490,9)
 (83.41463,8)
 (82.92683,7)
 (80.00000,6)
 (44.87805,5)
 (44.87805,4)
 (28.78049,3)
 (6.82927,2)
 (6.34146,1)
};
\addlegendentry{Pass}
\addplot+[fill=reac!75,draw=white,line width=0.25pt] coordinates {
 (4.87805,11)
 (7.84314,10)
 (7.84314,9)
 (9.26829,8)
 (6.82927,7)
 (6.34146,6)
 (24.39024,5)
 (10.73171,4)
 (41.46341,3)
 (48.29268,2)
 (49.26829,1)
};
\addlegendentry{Partial}
\addplot+[fill=orange!35,draw=white,line width=0.25pt] coordinates {
 (0.00000,11)
 (0.00000,10)
 (0.00000,9)
 (0.00000,8)
 (0.00000,7)
 (0.00000,6)
 (0.00000,5)
 (0.00000,4)
 (0.00000,3)
 (3.41463,2)
 (2.43902,1)
};
\addlegendentry{Near}
\addplot+[fill=orange!75!black,draw=white,line width=0.25pt] coordinates {
 (2.92683,11)
 (2.45098,10)
 (2.94118,9)
 (3.90244,8)
 (3.41463,7)
 (1.46341,6)
 (8.29268,5)
 (13.17073,4)
 (6.82927,3)
 (0.00000,2)
 (0.00000,1)
};
\addlegendentry{Fail-close}
\addplot+[fill=flowc!38,draw=white,line width=0.25pt] coordinates {
 (1.95122,11)
 (1.47059,10)
 (1.96078,9)
 (3.41463,8)
 (6.82927,7)
 (12.19512,6)
 (22.43902,5)
 (31.21951,4)
 (22.92683,3)
 (41.46341,2)
 (41.95122,1)
};
\addlegendentry{Fail}
\end{axis}
\end{tikzpicture}
\Description{Recorded pass, partial, near, fail-close and fail shares for eleven model configurations.}
\caption{Recorded grade distributions normalized by each configuration's evaluated task count. Non-pass categories are descriptive and are not uniformly calibrated measures of financial-error severity.}
\label{fig:outcomes}
\end{figure*}

